Ploutos: Towards interpretable stock movement prediction with financial large language model

Recent advancements in large language models (LLMs) have opened new pathways for many domains. However, the full potential of LLMs in financial investments remains largely untapped. There are two main challenges for typical deep learning-based methods for quantitative finance. First, they struggle to fuse textual and numerical information flexibly for stock movement prediction. Second, traditional methods lack clarity and interpretability, which impedes their application in scenarios where the justification for predictions is essential. To solve the above challenges, we propose Ploutos, a novel financial LLM framework that consists of PloutosGen and PloutosGPT. The PloutosGen contains multiple primary experts that can analyze different modal data, such as text and numbers, and provide quantitative strategies from different perspectives. Then PloutosGPT combines their insights and predictions and generates interpretable rationales. To generate accurate and faithful rationales, the training strategy of PloutosGPT leverage rearview-mirror prompting mechanism to guide GPT-4 to generate rationales, and a dynamic token weighting mechanism to finetune LLM by increasing key tokens weight. Extensive experiments show our framework outperforms the state-of-the-art methods on both prediction accuracy and interpretability.

==> kdd_sections/abstract.tex <==
\begin{abstract}
Recent advancements in large language models (LLMs) have opened new pathways for many domains. However, the full potential of LLMs in quantitative investment remains largely untapped. Traditional quantitative finance methods often suffer from a lack of transparency and explainability, hindering their adoption in decision-making processes where understanding the rationale behind predictions is crucial. Furthermore, traditional human-derived strategies are not easily amalgamated with advanced data-driven approaches, creating a gap between experiential wisdom and computational robustness. To address these challenges, we introduce PloutosGPT, a novel finance large language model (LLM) tailored for quantitative investment, which pioneers a unique training methodology that can dynamically incorporating insights from diverse quantitative strategy experts, both sentiment and technical analysis, by evaluating and aligning with their prediction accuracy. This adaptivelearning process enables PloutoGPT to selectively integrate the strengths of varied strategies, which could ensure optimal performance across different market conditions.
Furthermore, this training strategy not only facilitates the seamless combination of textual and numerical data but also provides clear, interpretable rationales for its predictions, demystifying the decision-making process. Extensive experiments show the effectiveness and interpretability of our proposed models. The code will be published after the acceptance of this paper.
	
% 	\let\thefootnote\relax\footnotetext{$^*$Corresponding Author.}
%     \addtocounter{footnote}{-1}\let\thefootnote\svthefootnote
\end{abstract}

==> kdd_sections/acknowledgements.tex <==

\section*{Acknowledgments}

The preparation of these instructions and the \LaTeX{} and Bib\TeX{}
files that implement them was supported by Schlumberger Palo Alto
Research, AT\&T Bell Laboratories, and Morgan Kaufmann Publishers.
Preparation of the Microsoft Word file was supported by IJCAI.  An
early version of this document was created by Shirley Jowell and Peter
F. Patel-Schneider.  It was subsequently modified by Jennifer
Ballentine, Thomas Dean, Bernhard Nebel, Daniel Pagenstecher,
Kurt Steinkraus, Toby Walsh, Carles Sierra, Marc Pujol-Gonzalez,
Francisco Cruz-Mencia and Edith Elkind.


==> kdd_sections/author.tex <==

% KDD author
% \author{Hanshuang Tong}
% \orcid{0000-0002-7443-128X}
% \affiliation{%
%   \institution{Microsoft Corporation}
%   \city{Beijing}
%   \country{China}}
% \email{hanstong@microsoft.com}

% \author{Jun Li}
% \affiliation{%
%   \institution{Microsoft Corporation}
%   \city{Beijing}
%   \country{China}}
% \email{junli1@microsoft.com}


% \author{Ming Gong}
% \authornote{Corresponding Author}
% \affiliation{%
%   \institution{Microsoft Corporation}
%   \city{Beijing}
%   \country{China}}
% \email{migon@microsoft.com}

% \author{Dongmei Zhang}
% \affiliation{%
%   \institution{Microsoft Corporation}
%   \city{Beijing}
%   \country{China}}
% \email{dongmeiz@microsoft.com}

% \author{Qi Zhang}
% \affiliation{%
%   \institution{Microsoft Corporation}
%   \city{Beijing}
%   \country{China}}
% \email{zhang.qi@microsoft.com}

% ACL author

\author{First Author \\
  Affiliation / Address line 1 \\
  Affiliation / Address line 2 \\
  Affiliation / Address line 3 \\
  \texttt{email@domain} \\\And
  Second Author \\
  Affiliation / Address line 1 \\
  Affiliation / Address line 2 \\
  Affiliation / Address line 3 \\
  \texttt{email@domain} \\}

==> kdd_sections/conclusion.tex <==
\section{CONCLUSION}
With the advancement of LLMs, people are gradually recognizing their potential in financial market~\cite{li2023large,wu2023bloomberggpt,zhang2023instruct}. In this work, we explored the feasibility of using LLMs to construct a assistant that can generate interpretable decision making rationals for stock movement prediction. Specifically, we first explore different strategies to analyze the multi-model stock related data for stock movement prediction from different perspectives. Then we propose PloutosGPT, which introduces an novel training approach called learning to rank rationales that designed to dynamically incorporate insights from diverse quantitative strategy experts, encompassing both sentiment and technical analysis. By calibrating against their predictive accuracies, PloutosGPT refines its capacity to selectively synthesizing the advantages of various strategies, thereby ensuring sustained superior performance under fluctuating market scenarios. Extensive experiments shows that our method can perform well under different conditions, reinforcing its practical applicability.




==> kdd_sections/ethical.tex <==
\section*{Ethical Statement}

There are no ethical issues.

==> kdd_sections/experiments.tex <==
\section{EXPERIMENTS}
Our experiments are designed to investigate the following research questions:

\begin{itemize}  
  \item \libertinebold{RQ}\textbf{1}: How does PloutosGPT perform compared with current LLMbased and traditional prediction models? 
  \item \libertinebold{RQ}\textbf{2}: How do the different components in PloutosGPT affect its effectiveness?  
  \item \libertinebold{RQ}\textbf{3}: Does the generated interpretable decision making rationales consistent with fact?
\end{itemize}


\subsection{Experiment Settings}

\subsubsection{Data}
In this study, we utilize the classic StockNet dataset for stock movement prediction to train and evaluate the performance of PloutosGPT~\cite{xu2018stock}. The dataset comprises 88 high-volume trading stocks from the S\&P 500 index listed on the NYSE and NASDAQ exchanges. Each of stock contains price data obtained from Yahoo Finance and related tweets data extracted using regular expression queries based on NASDAQ ticker symbols for each day (except for weekends and public holidays). Then a 5-day rolling window is utilized to produce data samples along the series of trading days. Samples are labeled as either positive or negative based on the percentage change in closing price, with increases of 0.55\% or more labeled as positive and decreases of 0.5\% or more labeled as negative, in order to generate an equitably partitioned dataset of 26,614 samples (49.78\% positive and 50.22\% negative). Following Xu and Chen~\cite{xu2018stock}, we split the dataset into distinct sets for training (01/01/2014 to 31/07/2015), validation (01/08/2015 to 30/09/2015), and testing (01/10/2015 to 01/01/2016) in a 7:1:2 ratio. 

\subsubsection{Evaluation Metric}
Since PloutosGPT aims to predict price movement for a given target day, $i.e.,$ a binary classification problem, we adopt accuracy, F1 score, and the Matthews Correlation Coefficient (MCC, sourced from sklearn's implementations\footnote{https://scikit-learn.org}) for classification performance. We employ MCC due to its robustness and unbias evaluation of classifier performance regardless of data imbalance as it considers all quadrants of the confusion matrix: 

\begin{equation}
\numberthis 
\label{eq:p2}
\text{MCC} = \frac{tp \cdot tn - fp \cdot fn}{\sqrt{(tp + fp)(tp + fn)(tn + fp)(tn + fn)}}
\end{equation}


\subsubsection{Baselines}
We compare PloutosGPT with the below baselines spanning both traditional model based and LLM based methods.

\noindent{$\textbf{Traditional Methods}$}: These methods uses traditional small scale neural network such as time-series, graph based and others. 

\begin{itemize}  
\item \textbf{RAND}: A naive baseline through random guessing of price movements, serving as a stochastic approach to predict price fluctuations.

\item \textbf{ARIMA}~\cite{brown2004smoothing}: A time series model that adopts Autoregressive architecture that incorporate features such as Moving Average
to forecast future prices.

\item \textbf{Adv-LSTM}~\cite{selvin2017stock}: An advanced LSTM model with adversarial training strategy. 

% \item \textbf{TSLDA}: Topic Sentiment Latent Dirichlet Allocation model, which is a generative model that incorporates both sentiment analysis and topic modeling techniques on social media~\cite{nguyen2015topic}.

\item \textbf{HAN}~\cite{hu2018listening}: A hierarchical attention mechanism to intricately encode textual information both within a single day and across consecutive days.

\item \textbf{StockNet}~\cite{xu2018stock}: A hybrid model that combines a Variational Autoencoder with hierarchical attention mechanisms to encode textual data, and a sequential approach for modeling price features. 

\item \textbf{HATS}~\cite{kim2019hats}: A Hierarchical Graph Attention Network that adopts a novel multi-graph approach to weigh the diverse interconnections among stocks, utilizing only historical price data to inform its attention-based hierarchical structure.

\item \textbf{DTML}~\cite{nguyen2015topic}: A attention-based model that leverage correlations between stocks to improve the prediction accuracy..

\end{itemize}

\noindent{$\textbf{LLM Based Methods}$}: These methods leverage either zero shot or few-shot ability of large language model to predict the stock movement. 

\begin{itemize}  
\item \textbf{LLAMA2}~\cite{touvron2023llama}: A open source large language model developed by Meta AI, which outperforms many other open-source language models on multiple external benchmarks. 

\item \textbf{GPT4}~\cite{achiam2023gpt}: Developed by OpenAI, GPT4 is a multimodal large language model that shows incredible performance ability in diverse domain with its zero shot ability.

\item \textbf{FinMA}~\cite{xie2023pixiu}: A financial large language model (LLM) fine-tuned to follow natural language instructions, enhancing its performance in many downstream financial tasks. 

\end{itemize}



\begin{table*}[]
\centering
\caption{A comparison of prediction accuracy and MCC between PloutosGPT and other baselines.}
\label{tab:t15}
\begin{tabular}{lllll}
\bottomrule[1pt]
                    & \textbf{Model}    & \textbf{Accuracy} & \textbf{MCC} & \textbf{F1}    \\
\hline
Traditional Methods & RAND        & 50.89    & -0.002 & 0.502  \\
                    & ARIMA       & 51.42    & -0.021 & 0.513  \\
                    & HATS         & 56.21    & 0.117& 0.560 \\
                    & Adv-LSTM     & 57.20    & 0.148 & 0.570\\\
                    & DTML    & 57.44    & 0.191  & 0.571 \\
                    & HAN         & 57.64    & 0.052& 0.572  \\
                    & StockNet    & 58.23    & 0.081  & 0.575 \\
\hline
LLM-Based Methods   & LLAMA2 - 7B       & 50.92    & -0.002 & 0.503 \\
                    & GPT4      & 52.16    & 0.027 & 0.519  \\
                    & FinMA - 7B       & 56.43    & 0.107 & 0.562  \\
                    & \textbf{PloutosGPT - 7B}     & \textbf{59.17}   & \textbf{0.166} & \textbf{0.589}\\
\bottomrule[1pt]
\end{tabular}
\end{table*}





\subsubsection{Training settings}
We conduct all experiments on 8 Tesla V100 GPU. To get the best performance of PloutosGPT, we apply grid search to get best batch size (128) and learning rate (2e-06). Adam is used as the optimizer and we leverage our framework to fine-tune from LLAMA2 for 1 epochs on all datasets. It takes about 18.5 and 1 hours to train and test on StockNet datasets, respectively.  As for other baselines, there are two conditions: i) where official implementations or open-source libraries corresponding to the baseline models existed, the same hyperparameters are applied to ensure a fair comparison. ii) Where no such implementations were available,  the algorithms were re-implemented with utmost fidelity to the settings provided in the original papers.



\subsection{Performance Comparison (\libertinebold{RQ}\textbf{1})}

We compare the stock movement prediction performance of various methods including both traditional and LLM based methods. The evaluation results against baseline methods are presented in Table \ref{tab:t15}. From the figure and table, we draw the following conclusions: 1) Our method significantly outperforms both traditional and LLM based methods, verifying the superiority of tuning LLMs via our proposed training framework. PloutosGPT successfully unlocks the text and numerical data understanding capabilities of LLMs for stock movement prediction task. 2) Traditional CNN,LSTM or graph based models such as ARIMA, HATS and others perform worse than PloutosGPT, implying the potential of leveraging language model to process and understand multi-mode stock related data. 3) The zero shot ability of LLAMA2 and GPT4 perform similarly to random guessing (ACC$\simeq 0.5$). However, the LLMs trained via diverse strategy experts data and learning to rank rationale strategy achieves significant improvements. These results demonstrate a considerable gap between stock movement prediction and language tasks, showing the importance of using stock related data for tuning on LLMs. 4) Financial large language model FinMA-7B trained with StockNet training set yield inferior performance than PloutosGPT, indicating purely tuning LLM with stock related instruction data cannot get optimal performance for stock movement prediction task.


\begin{table}[]
\centering
\caption{Performance of PloutosGPT variants on StockNet dataset, showing every component makes an important contribution to the excellent performance.}
\label{tab:t16}

\begin{tabular}{llll}
\bottomrule[1pt]
\textbf{Model}    & \textbf{Accuracy} & \textbf{MCC} & \textbf{F1}    \\
\hline
PloutosGPT-SA        & 53.92    & 0.062 & 0.528  \\
PloutosGPT-TA         & 55.96    & 0.119 & 0.537  \\
PloutosGPT-LRR          & 56.21    & 0.117 & 0.560 \\
\hline
\textbf{PloutosGPT}          & \textbf{59.17}    & \textbf{0.166} & \textbf{0.589} \\

\bottomrule[1pt]
\end{tabular}
\end{table}


\subsection{Ablation Study (\libertinebold{RQ}\textbf{2})}

To evaluate the contribution of PloutosGPT's different components, we compare against several variants: 
\begin{itemize}
    \item \textbf{PloutosGPT-SA}: PloutosGPT without the sentiment analysis expert, which makes decisions just based on the numerical technical analysis. 
    \item \textbf{PloutosGPT-TA}: PloutosGPT without the technical analysis expert, which makes decisions just based on the news sentiment analysis. 
    \item \textbf{PloutosGPT-LRR}: PloutosGPT without the learning to rank the rationales training strategy, which instruction tuning process based on the input from diverse experts and output from stock movement. 
\end{itemize}

The results are shown in Table \ref{tab:t4}. PloutosGPT-SA only achieves a level of prediction accuracy on par with ALSTM and Adv-LSTM, and is worst among all the variants, again indicating the importance of text data. Similar to the performance of Stocknet, PloutosGPT-TA has a relatively high Acc. but a low MCC, suggesting texts are particularly helpful to predict on one side of the binary classification. By modeling both text data and stock relationships, PloutosGPT-LRR reaches a good result. Finally, better performance achieved when diverse stratgy expert pool and learning to rank rationales are introduced into the network. In summary, the ablation studies conclusively demonstrate that each component within the PloutosGPT architecture is important, and as a result the full model with all components achieves the best performance.      

\subsection{Faithfulness of Interpretablity (\libertinebold{RQ}\textbf{3}) - Placeholder }

Table 3 shows an example combination of 10 alphas generated by our framework, evaluated on the CSI300 constituent stock set. Most of the alpha pairs in this specific set have mutual IC values over 0.7. Previous work [10][27] considered this to be too high for the
individual alphas to be regarded as diverse, yet these alphas are able to work well in a synergistic manner. For example, the alphas 2 and 6 have a mutual IC of 0.9746, thus traditionally considered too similar to be useful cooperatively. However, the combination 0.093172 − 0.071636 achieves an IC of 0.0458 on the test set, even higher than the sum of the respective ICs, showing the synergy effect. Also, although alpha #1 only has an IC of 0.0011, it still plays a vital role in the final combination. Once we remove alpha #1 from the combination and re-train the combination weights on the remaining set, the combination’s IC drops to merely 0.0447. The two observations above show that neither the single alpha IC nor the mutual IC between alpha pairs is a good indicator of how well the combined alpha would perform, answering Q3. One possible explanation for these phenomena is that: Although traditionally these alphas are similar due to the high mutual IC, some linear combinations of the alphas could point to a completely different direction from the original ones in the vector space. Consider two unit vectors in a linear space: The more similar these two vectors are, the less similar either of these vectors is to the difference between the two vectors, because as the two unit vectors get closer, the difference vector approaches perpendicular to both of the original vectors

% \subsection{Case Study - Placeholder}

% Table 3 shows an example combination of 10 alphas generated by our framework, evaluated on the CSI300 constituent stock set. Most of the alpha pairs in this specific set have mutual IC values over 0.7. Previous work [10][27] considered this to be too high for the
% individual alphas to be regarded as diverse, yet these alphas are able to work well in a synergistic manner. For example, the alphas 2 and 6 have a mutual IC of 0.9746, thus traditionally considered too similar to be useful cooperatively. However, the combination 0.093172 − 0.071636 achieves an IC of 0.0458 on the test set, even higher than the sum of the respective ICs, showing the synergy effect. Also, although alpha #1 only has an IC of 0.0011, it still plays a vital role in the final combination. Once we remove alpha #1 from the combination and re-train the combination weights on the remaining set, the combination’s IC drops to merely 0.0447. The two observations above show that neither the single alpha IC nor the mutual IC between alpha pairs is a good indicator of how well the combined alpha would perform, answering Q3. One possible explanation for these phenomena is that: Although traditionally these alphas are similar due to the high mutual IC, some linear combinations of the alphas could point to a completely different direction from the original ones in the vector space. Consider two unit vectors in a linear space: The more similar these two vectors are, the less similar either of these vectors is to the difference between the two vectors, because as the two unit vectors get closer, the difference vector approaches perpendicular to both of the original vectors

==> kdd_sections/intro.tex <==


\section{INTRODUCTION}

The prospect of predicting stock market trends has continually intrigued both academics and investors for a long time, and it is still challenging due to the volatile nature of financial markets and multimodal features related to stock price~\cite{adam2016stock}, such as textual features (e.g., news, tweets) and time-series numerical features (e.g. price sequence, volumes sequence)~\cite{anthony1992association,kohara1997stock,neal1998measures}. 
In practice, researchers focus more on predicting stock movement (whether the stock price movement will increase or decrease) rather than attempting to predict the precise stock price values, which are widely recognized as a inherently unpredictable task.~\cite{walczak2001empirical}.

Existing quantitative methods can be divided into two tracks: traditional  deep model based and large language model (LLM) based track. Traditional quantitative deep model based methods have attempted to unify stock social media texts and price signal by LSTM-based, transformer-based and graph-based deep models~\cite{feng2018enhancing,gao2023stockformer,sawhney2020deep}. However, these deep learning models in quantitative finance are often criticized for their opacity and lack of explainability issue. A common area of focus for quantitative investment is the mining of good alphas which is a important financial feature or a function with predictive power over excess return or risk, but incorporating these alpha features into deep learning models complicates risk assessment and management for investors due to difficulties in understanding how the underlying factors drive the models' prediction. For the LLM based track, some recent work attempts to predict the stock based on the sentiment score labeled by LLM or incorporate limited news and price information into LLM training ~\cite{chen2023chatgpt,xie2023pixiu}. Nevertheless, they also lack of explainability and the diversified strategy such as technical analysis with alpha features and other human expert derived strategy for different market situations is not considered. 


\begin{figure*}[htb]
	\centering
	\includegraphics[width=\linewidth]{diagram/inspiration_v1.pdf}
	\caption{Comparison of Quantitative Methods}
	\label{fig:inspiration}
\end{figure*}

Our insight of solving the explainability and strategy diversification problems hinges upon the idea of fully exploring the extensive ability of large language models (LLMs) to interpret and analyze the multimode data, and generate rationales learned from diverse experts. Specifically, we first borrow the concept from a common economics phenomenon that \textit{the rearview mirror is always clearer than the windshield}~\cite{Berkshire1991}, which indicate that analyze the rationales of past cases is always easier than predicting the future. Each time there's a movement in stock prices, we can always find economic experts using their strategies to account for the price variations. Their insights from hindsight or tactics might not be used directly to predict the future price, but we can still learn from the those experts who have high prediction accuracy, tailoring these to different market situations to improve our forecast accuracy for next predictions. Fig.~\ref{fig:inspiration} shows the basic idea of our method, by leveraging the interpretative and analytical capabilities of large language model to process multimodal data from diverse strategy experts, it can adaptively learn and evolve their strategies to accommodate varying market conditions, and generate convincible decision making rationales. 

The above analysis shows the prospects of introducing large language model with diverse experts into quantitative investment. However, it may also bring in the following problems. Firstly, the stock multimode features contains time series derived from various alpha formulas. The capability of large language model to interpret and analyze the time series numeric data from multiple domains remains unknown. Recent studies have attempted to frame time series forecasting as next-token prediction in text by encoding time series as a string of numerical digits~\cite{gruver2023large}. Nevertheless, the numerical features of stock time series data do not conform to this paradigm.  Secondly, the correlation between news events and their effect on stock valuations is well-established. The influence exerted by tweets is heterogeneous, reliant on the inherent value of the content—ranging from breaking news to trivial commentary. Aggregating this diverse news requires sophisticated endeavor. Thirdly,  the predictive accuracy of strategy experts can vary considerably across different stock situations. Hence, an adaptive framework that effectively harnesses the insights of the most suitable experts for any given stock situation is needed.

To address the above challenges, we propose PloutosGPT that equipped with learning to rank rational (LRR) training strategy to adaptively learn knowledge from diverse strategy experts.  To summarize, the main contributions of this work are as follow: 

\begin{itemize}

% \item PloutosGPT is the first quantitative investment model that generate explainable stock prediction

\item We prompt and tuning a large language model for explainable quantitative investment, demonstrating the LLM's capability in stock prediction task.

\item We propose PloutosGPT that could incorporate insight from diverse experts, and generate convincing decision-making rationales with leverage rank rationale (LRR) training strategy.

\item We enhance the ability of large language models to interpret and analyze multimodal data, particularly numeric time series data derived from various alpha formulas.
\end{itemize}  













==> kdd_sections/methodology.tex <==
\begin{figure*}[htb]
	\centering
	\includegraphics[width=\linewidth]{diagram/frameworkv2.pdf}
	\caption{PloutosGPT internal working pipeline: When predicting the price movement of a given stock, the diverse strategy experts pool would first leverage its diverse experts to gather and analysis the stock related feature with his strategy. Then, the ploutosGPT trained with LRR strategy would generate bullish and bearish rationales to make final decision based on the market condition and opinions from diverse expert.}
	\label{fig:framework}
\end{figure*}

\section{METHODOLOGY}

In this section, we first give an overview of the framework of PloutsGPT, followed with a detailed explanation of each component. The intuition of framework of PloutsGPT could be considered as an ensemble learning approach that leverage large language model to adaptively leverage different methods to predict the stock price. As shown in Fig.~\ref{fig:framework}, the framework of PloutosGPT includes two primary components. The diverse strategy experts pool span a wide range of experts, including sentiment and technical analysis, each possibly utilizing a Large Language Model (LLM), algorithms, or unique strategies to analyze the stock related information from a specific perspective. In the subsequent training stage,  a frozen LLM is employed to initially deduce the ranked rationales behind stock price fluctuations for training set generation. Leveraging this curated training dataset, PloutosGPT acquires the capability to articulate coherent and explainable investment strategy.

\subsection{Diverse Strategy Expert Pool}
To fully utilize strategy from different experts in financial market, the diverse strategy expert pool is designed to produce diversified ensemble experts. It constitutes a range of experts whose strategies are based on different principles and data sources. The pool includes a sentiment analysis expert, a technical analysis expert, and a human financial expert that can customize human strategy. By integrating insights from these experts, PloutosGPT can leverage a broad spectrum of knowledge and techniques to inform its predictive capabilities.

\subsection{Sentiment Analysis Expert}
In this section, we would introduce how we leverage only the sentiment information to predict the stock price. Many existing research has shown the effectiveness of social media as a promising tool for stock market prediction~\cite{si2013exploiting,si2014exploiting}. However, there are still two major challenges. i) Existing large language model usually not specifically fine-tuned for stock price from sentiment analysis perspective; ii) how to aggregate news or tweets into stock price movement signals since different events have different impact for stock price. To address these two challenges and fill the gap, we explore the following ways by classified by whether stock movement signal is used to train our model: unsupervised, supervised and supervised\&unsupervised sentiment-based stock prediction. 


\begin{table}[h]
	\centering
	\caption{Unsupervised sentiment analysis based prompt}
	\label{tab:t2}
\begin{tabular}{p{8cm}}
\bottomrule
\multicolumn{1}{c}{\textbf{Instruction Input}} \\
\hline
Instruction: What is the sentiment of this news/tweet? \\
Please choose an answer from \{Negative/Neutral/Positive\}. \\
Input: Mr Ashley sold a 43pc stake in the company for more than pounds 900m at the time of the float. \\
Answer: \\
\hline
\multicolumn{1}{c}{\textbf{Instruction Output}} \\
\hline
Negative \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection{Unsupervised method}
Our \emph{unsupervised} sentiment-based stock prediction method simply predicts the stock movement with average aggregated sentiment score of news. We collect the financial sentiment analysis datasets and convert it into instruction tuning dataset with prompt showing in Table \ref{tab:t2}. We first explore which sentiment analysis dataset are especially suitable for stock prediction task. We experiment with a number of datasets including 1) FIQA-SA~\cite{maia201818}: sentiment analysis on FiQA; 2) NWGI~\cite{chu2023data}: news with GPT instruction; 3) BTSA~\cite{kaggleBitcoinTweets}: BTC tweets sentiment; 4) TNFS ~\cite{zeroshottwitterfinancialnewssentiment}: twitter financial news sentiment. The above datasets are selected based on the diversity between different assets and news type, which is a crucial step to ensure that the models are trained on a wide-ranging corpus of finance information, promoting robustness and adaptability in practical application. The constructed sentiment instruction data are used to directly tuning LLM. Here we use the common used open source large language model Llama2 as backbone of our LLM. The performance of those dataset sets are evaluate by StockNet dataset (see section 4 for details of this evaluation set). Once the sentiment analysis model is trained, we use it to label each news from the past 5 days ($\mathcal T=5$) of a particular stock as positive, negative, or neutral. The stock price movement on the target day $d$ is simply calculate as the average of sentiment scores. Here, a positive sentiment score suggests an increase, while a negative score suggests a decrease prediction for the stock price.  Table 4 shows the comparison of the impact for stock movement prediction task over different datasets. Among all the options, the \emph{unsupervised} method combining all the datasets performs the best, which is reasonable since this method consists of most diversified and robustness data for sentiment analysis. Besides,  the accuracy of stock market predictions using sentiment scores calculated by this unsupervised method hovers around 50\%, which is not particularly high. This indirectly suggests that while the sentiment of these news articles does have a positive correlation with stock prices, there is also a lot of noise within the news itself. We need to develop better methods to aggregate this news.

\begin{table}[]
	\centering
	\caption{Comparison of the impact for stock movement prediction task over different datasets. The definition of MCC are introduced in section A. The Unsup. method denote that the combined dataset including both FIQA-SA, NWGI, BTSA, TNFS datasets. }
	\label{tab:t1}
\begin{tabular}{lllll}
\bottomrule
\textbf{Dataset}                & Accuracy          & MCC           &  &  \\
\hline
FIQA-SA~\cite{maia201818}                & 0.529          & 0.032          &  &  \\
NWGI~\cite{chu2023data}                   & 0.524          & 0.014          &  &  \\
BTSA~\cite{kaggleBitcoinTweets}                   & 0.525          & 0.043          &  &  \\
TNFS~\cite{zeroshottwitterfinancialnewssentiment}                   & 0.511          & -0.021         &  &  \\
\hline
Unsup. & \textbf{0.532} & \textbf{0.052} &  &  \\
\bottomrule


\end{tabular}
\end{table}


% \begin{tabular}{l|c|c|c}
% \hline
% \multicolumn{1}{c|}{\textbf{Model}} & \multicolumn{1}{c|}{\textbf{F1$\uparrow$}} & \multicolumn{1}{c|}{\textbf{Accuracy$\uparrow$}} & \multicolumn{1}{c|}{\textbf{MCC$\uparrow$}} \ \hline
% RAND & 5.028e-5 & 5.098e-5 & -0.002 ± 1e-3 \
% & 5.131e-3 & 5.141e-3 & -0.0212e-3 \ \hline
% Selvin et al. (2017) & 5.295e-2 & 5.305e-2 & -0.0047e-2 \ \hline
% RandForest (Venkata Sasank Pagolu, 2016) & 5.272e-3 & 5.312e-3 & 0.0134e-3 \ \hline
% TSLDA (Nguyen and Shirai, 2015) & 5.396e-3 & 5.416e-3 & 0.0657e-3 \ \hline
% HAN (Hu et al., 2018) & 5.724e-3 & 5.764e-3 & 0.0525e-3 \ \hline
% StockNet - TechnicalAnalyst (Xu and Cohen, 2018) & 0.572$^{+}$ & 0.546$^{-}$ & 0.550$^{-}$ & 0.017$^{-}$ \
% StockNet - FundamentalAnalyst (Xu and Cohen, 2018) & 0.582$^{-}$ & 0.072$^{-}$ \ \hline
% StockNet - IndependentAnalyst (Xu and Cohen, 2018) & 0.559$^{+}$ & 0.573$^{-}$ & 0.575$^{-}$ & 0.037$^{+}$ & 0.056$^{-}$ \
% & 0.562$^{-}$ \ \hline
% FA StockNet - DiscriminativeAnalyst (Xu and Cohen, 2018) \ \hline
% StockNet - HedgeFundAnalyst (Xu and Cohen, 2018) & 0.575$^{+}$ & 5.602e-3 & 0.582$^{+}$ & 5.622e-3 & 0.081$\pm$ & 0.1176e-3 \ \hline
% HATS (Kim et al., 2019) \ \hline
% Chen et al. (2018) & 5.307e-3 & 5.327e-3 & 0.0939e-3 \ \hline
% Adversarial LSTM (Feng et al., 2019a) & 0.570$^{-}$ & 0.572$^{-}$ & 0.148$^{-}$ \ \hline
% MAN-SF (This work) & 6.052e-4 & 6.082e-4 & 0.1956e-4 \ \hline
% \end{tabular}

\begin{table}[h]
	\centering
	\caption{Supervised sentiment analysis based prompt}
	\label{tab:t3}
\begin{tabular}{p{8cm}}
\bottomrule
\multicolumn{1}{c}{\textbf{Instruction Input}} \\
\hline
Instruction: Predict the MSFT's price movement for the 2015-06-10 based on the following tweets. \\
Please choose an answer from Up or Down.\\
Input: From 2015-06-05 to 2015-06-09, company related news during this period are listed below: \\
2015-06-08: game-changers announced at microsoft \\
2015-06-09: microsoft lumia sales tops apple in pakistan \\
2015-06-09: msft - are the days of subsidized 200 smartphones nearing an end? \\
Answer: \\
\hline
\multicolumn{1}{c}{\textbf{Instruction Output}} \\
\hline
Up \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection{Supervised method}
Our \emph{supervised} sentiment-based stock prediction method builds upon the recent success of long context length encoding ability of large language model. Aggregating and debasing the impacts of various news on stock trends has always been challenging. Historically, models constrained by the length of input would usually convert news into sentiment scores or construct graph networks for deep learning models~\cite{si2014exploiting, xu2021rest}. However, we can now use LLM to enable the encoding of extensive news content, allowing the model to filter valuable information and analyze the weight of different news to make a final prediction. To elaborate, we construct the instruction with the prompt shown in Table \ref{tab:t2}, which takes the news text from the five days preceding the target day as input, and the stock price on the target day as the prediction label.
Similarly, we adopt llama2 as our base model for training and build our supervised method. Additionally, we attempted to combine the 'unsup' instruction set to integrate both supervised and unsupervised methods. Table \ref{tab:t4} shows the prediction results on StockNet for different methods. The results indicate that the combined 'sup \& unsup' method performs the best, which also demonstrates the effectiveness of both our supervised and unsupervised approaches.


\begin{table}[]
	\centering
	\caption{Comparison of the impact for stock movement prediction task over different methods. }
	\label{tab:t4}
\begin{tabular}{lllll}
\bottomrule
\textbf{Method}                & Accuracy          & MCC           &  &  \\
\hline
Unsupervised                & 0.532          & 0.054          &  &  \\
Supervised                 & 0.528          & 0.043         &  &  \\
\textbf{Sup.\& Unsup.}          & \textbf{0.539}          & \textbf{0.062} &  & \\
\bottomrule
\end{tabular}
\end{table}


\begin{figure*}[htb]
	\centering
	\includegraphics[width=\linewidth]{diagram/technical_expert_v1.pdf}
	\caption{The idea of number to text alignment used by technical analysis expert.}
	\label{fig:technical_expert}
\end{figure*}
 
\subsection{Technical Analysis Expert}



The technical analysis expert focuses on analyzing historical price and volume data to identify market trends and patterns. With the success of LLMs for time series stems from their ability to naturally represent multimodal distributions, some methods explored ways to frame time series forecasting as next-token prediction in text~\cite{gruver2023large}. However, there are still two limitations. Firstly, the existing method focus more on the single feature time series prediction. However, the alpha generated features in stock prediction are time series data cross different domain which we called cross-feature time series prediction in Fig.~\ref{fig:technical_expert}. Second, the existing time series prediction method lacks of explainability, which does not fully use the natural language generation ability of large language model. Our idea of solving the above challenges hinge upon the idea of fully use incorporates large language models(LLM) as a mediator between different alpha features (time series features) and its explanation (text features). We propose Number-to-Text Alignment (N2I-Align), a method for cross feature time series forecasting, by integrating the domain specific explaining texts (as shown in Fig.~\ref{fig:technical_expert}), we can convert this cross feature time series prediction task to next token prediction task. 

Specifically, for a given stock $s \in \mathcal S$, a target prediction date $d$, and price data in a period of days with fix windows size. We initially produce a set of cross-feature time series datasets by leveraging a selection of widely-recognized alphas. Here, we only adopt some common used alphas shown in Appendix \ref{tab:t4}. (Alpha mining are getting more popular recently, but they are not discussed in this work).  Following the generation process, the cross feature time series data would be rescaled to integer, and tokenized into sequences. It is noteworthy that prevalent tokenization methods, such as Byte Pair Encoding (BPE), may fragment individual numbers into subtokens that do not correspond to the original numerical values, thereby complicating subsequent arithmetic operations. For instance, under the tokenization of GPT-3, the number 63035422 would be partitioned into subtokens [630, 35, 422], with minor numerical adjustments potentially leading to vastly different tokenizations~\cite{liu2023goat}. Some strategies have been proposed to ensure each digit is tokenized separately by spacing them apart and using commas to segregate temporal data points within a series, yet this leads to an excessive consumption of token capacity~\cite{gruver2023large}. To circumvent these limitations, we utilize the LLaMA2 model, which intuitively tokenizes numbers into individual digits by default. At last, the technical expert leverage the number-to-text prompt to wrap cross feature tokenzied sequence and generate the instruction training data for LLM tuning. 

To evaluate the performance of the number-to-text-alignment, we carefully choose two popular time series baselines: 1) LLMTime~\cite{gruver2023large}: a single feature time series prediction method. Here we combine simply combine cross feature time series prediction sequences into one time series sequence; 2) LLMDate: following prompt in ~\cite{xie2023wall} which split time series features by date, we adopt similar prompt showing in appendix. We use the same base model and hyperparamters to evaluate the performance of the above prompts. As shown in Table \ref{tab:t9}, the performance of LLMTime is close to random, which indicates that the LLM is not good at cross feature time series prediction without meticulous task conversion. Besides, we find that N2I-Align performs the best, showing the effectiveness of number to text alignment. 

\begin{table}[]
	\centering
	\caption{Comparison of the impact for stock movement prediction task over different methods. }
	\label{tab:t9}
\begin{tabular}{lllll}
\bottomrule
\textbf{Method}                & Accuracy          & MCC           &  &  \\
\hline
Rand                & 0.506          & 0.002          &  &  \\
LLMTime                 & 0.511          & 0.028         &  &  \\
LLMDate                 & 0.534          & 0.082         &  &  \\
\textbf{N2I-Align}          & \textbf{0.559}          & \textbf{0.119} &  & \\
\bottomrule
\end{tabular}
\end{table}




% \subsubsection{Human Financial Expert}
% The Human Financial Expert encapsulates the wisdom and intuition of seasoned investment professionals. This component of the expert pool leverages the tacit knowledge of human experts, including insights from fundamental analysis, macroeconomic indicators, and market cycles. The key feature of this expert is its ability to contextualize financial data within a broader economic and financial framework, providing an additional layer of analysis that is often difficult to quantify but critical for making informed investment decisions.


\subsection{Learning to Rank and Reasoning}
The Learning to Rank (LRR) training strategy is the core component of PloutosGPT to produce explainable price movement prediction reasoning rationals, which could greatly help quant researchers' decision making process. Recently, the researchers area have emerging interest in explainable AI in Finance research in different dimensions~\cite{weber2023applications}. For example, some attempts focus on produce interpretable stock price predictors in the form of neuro-fuzzy rules~\cite{rajab2019interpretable,vlasenko2019novel}. Similarly,  et al.~\cite{yang2018explainable} have tried to provide interpretablity by leveraging attention-based neural network to assign importance to different news. Unfortunately, the interpretability of those existing methods heavily compromised by the learning phase of the neural network. To best of our knowledge, the LRR training strategy module in PloutosGPOT is the first method that can produce natural language rationals to interpretable stock movement prediction. Specifically, the LRR training strategy would generate a instruction tuning dataset for explainable exaplainable stock movement prediction. Overall, it consists of two steps: rational generation step and rationals combination step. In the first step,  as shown in image, we would prompt a strong frozen LLM (e.g. GPT-4) to summary both the bullish and bearish rationales for the price movement base on diverse experts input, and rank those rationales based on the prediction accuracy (Since the ground truth is given, the frozen LLM knows which rational make correct prediction). Then, the model would prompt to make the final decision based on the trade-off between bullish and bearish rationale. The intuition of the above prompts is to generation ranked rationals by learning weights to each expert's input based on the accuracy and relevance of their predictions in different market conditions. All of the above prompt are under the requirement that the model should not directly use the ground truth as the rationales, which echo our init motivation in section A that the researchers is more good at analyze the past given the result than predicting the future. Here in practice, we combine the above prompts into one prompt to save frozen LLM calling budget. 

In the rationals combination step, the generated rations and stock movment label and combined as the output of instrution training output, and the input and analysis from diverse experts are combined as the input. An example of the constructed instrcution dataset are showning in the appendix. 

Leveraging this curated training dataset, PloutosGPT thus become not just a black-box predictor but a sophisticated decision support tool that combines the strengths of diverse strategies and provides actionable insights with a clear justification for its predictions. 





==> kdd_sections/package.tex <==
% %%
% %% \BibTeX command to typeset BibTeX logo in the docs
\AtBeginDocument{%
  \providecommand\BibTeX{{%
    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}
\usepackage{booktabs} % For formal tables
\usepackage{algorithm}
\usepackage{algorithmicx} %format of the algorithm
\usepackage{graphics}
\usepackage{ifthen}
\usepackage{amsmath}
\usepackage{latexsym}
\usepackage{CJK}

\usepackage{ifthen}
\usepackage{caption}
\usepackage{enumerate}
\usepackage{amsmath}
\usepackage{caption}
\usepackage{enumerate}
\usepackage{graphicx}
\usepackage{float}
\usepackage{bookmark}
\usepackage{amsmath}
\usepackage{multirow}

\usepackage{algpseudocode}
\usepackage{amsmath}
\usepackage{balance}

\usepackage{subfig}
\usepackage{graphics}
\usepackage{caption}
\usepackage{enumerate}
\usepackage{amsmath}
\usepackage{caption}
\usepackage{verbatim}
\usepackage{graphicx}
\usepackage{float}
\usepackage{amsmath}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{booktabs}
\usepackage{amsmath}
\usepackage[hang,flushmargin]{footmisc}
\usepackage{caption}
\usepackage{bbold}
\usepackage{color}
\usepackage[normalem]{ulem}
\usepackage{arydshln}
\usepackage{svg}
\svgsetup{
	inkscapepath=i/svg-inkscape/
}
\svgpath{{svg/}}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newsavebox\CBox
\def\textBF#1{\sbox\CBox{#1}\resizebox{\wd\CBox}{\ht\CBox}{\textbf{#1}}}
\newcommand{\ze}[1]{\textcolor{red}{\emph{[ze: #1]}}}
\usepackage{newtxtext,newtxmath}

\usepackage{libertine}  
\usepackage[T1]{fontenc}  
\newcommand{\libertinebold}[1]{{\fontfamily{LinuxLibertineT-OsF}\fontseries{b}\selectfont #1}}  




==> kdd_sections/problem_formulation.tex <==
\section{PROBLEM FORMULATION}
We formulate the quantitative investment task in this paper as follows.
The goal is to learn stock price related information from both social media, specifically tweets, and past stock performance indicators to predict stock trends. The direction of a stock's movement is determined by comparing its adjusted closing prices over two consecutive trading days. This analysis is structured as a binary classification task, where the prediction revolves around whether the price of a particular stock will move up or down.


\subsection{Stock Prediction} 



For a given stock $s \in \mathcal S$, a target prediction date $d$, and related historical prices and  news data, we define stock movement prediction label over a period of $\mathcal T$ days as:

$$Y_{d}=
\begin{cases}
\numberthis 
\label{eq:p1}
0, & $$p_{d}^{c} < p_{d-1}^{c}$$\\
1, & $$p_{d}^{c} \geq p_{d-1}^{c}$$\\
\end{cases}$$

Here the $p_{d}^{c}$ represents the adjusted closing price in the target prediction date $d$~\cite{xu2018stock, sawhney2020deep}. The label $Y_{d}=$ is categorized as $0$ if there's a decrease in the adjusted closing price, and as $1$ indicate a rise in the adjusted closing price. 



==> kdd_sections/related_work.tex <==
\section{Related Work}\label{2}

\subsection{Stock Prediction with Deep Learning} Deep learning approaches have gained prominence for their capacity to model complex patterns in stock market data. It can be divided into several tracks: RNN Based, CNN Based, Transformer Based and Graph Based Models. Recurrent neural networks (RNNs) are favored for their proficiency in capturing sequential trends in stocks~\cite{li2018stock,qin2017dual}, with advancements like Long Short-Term Memory (LSTM) networks enhanced by adversarial training demonstrating superior performance in stock prediction~\cite{feng2018enhancing}. Moreover, CNN Based Models incorporating stock times series data as a set of input feature maps~\cite{hoseinzade2019cnnpred,lu2021cnn}. Furthermore, the emergence of transformer-based models, exemplified by StockFormers~\cite{gao2023stockformer}, showcases the effectiveness to extract latent representations of long short term stock states and asset relations. Recent efforts have also explored Graph-based deep learning models have been employed to analyze the interconnections among stocks, outperforming price-only models~\cite{sawhney2020spatiotemporal,kim2019hats,sawhney2020deep}. 


% \subsection{Stock Prediction with Sentiment Analysis} 
% The recent strides in natural language processing (NLP) have catalyzed the exploration of incorporating text data such as news, tweets, posts into stock movement prediction. Some attempts focus more on Certain investigations, such as the one conducted by Hu et al. (2018), have exclusively concentrated on textual data, employing sophisticated attention mechanisms within deep learning architectures to discern and leverage the most salient news narratives for forecasting stock prices. Meanwhile, alternative methodologies involve a bifurcated analytical process, where sentiment and other textual features are initially extracted and subsequently integrated with quantitative market data to enhance prediction models, as exemplified by the works of Li et al. (2017) and Jin et al. (2020). This symbiotic fusion of qualitative text analysis and quantitative modeling is poised to significantly augment the precision and robustness of stock movement forecasts.


\subsection{Stock Prediction with Large Language Model} 
The recent strides in large language model (LLM) have catalyzed the exploration of stock prediction application with LLM. Existing studies consists of several directions. Some studies focus solely on textual information. Lopez-Lira et al.~\cite{lopez2023can} demonstrate the correlation bewteen ChatGPT sentiment score and subsequent stock movement. Some researchers focus more on 
the numerical feature, Alpha-GPT is proposed as a new alpha mining paradigm by leveraging the power of large language models~\cite{wang2023alpha}. Others propose methods combine numerical and textual features, Xie et al.~\cite{xie2023pixiu,xie2023wall} directly prompt and fine-tune LLM to leverage both news and numerical features. Futhormore, Chen et al.~\cite{chen2023chatgpt} explore the relationship between stock by analyzing the textual information by ChatGPT. However, these techniques fall short of exploring the interpretablity ability of LLM, thereby limiting their application potential.


\subsection{Language Model for Time Series Prediction} 
There have been several studies to integrate language models (LMs) with time series data prediction. In the early time, most researchers were built open fine-tuning small scale transformer-like models. For example, FPT provide a unified framework to fine-tune BERT models with diverse time series analysis tasks~\cite{zhou2023one}. Similarly, Meta-Transformer is proposed to encode multimodel data including time-series~\cite{zhang2023meta}. Recently, with the success of large language model in many domains,  PromptCast first converts the times series prediction task as question answering task with prompting. However, it have not bridging the gap between time series prediction and next token prediction in language model~\cite{xue2023promptcast}. By encoding time series as a string of numerical digits, LLMTIME successfully frame time series forecasting as next-token prediction in text. The existing paper focus more on the single-variable time series prediction, which does not adequately address the complexities of multi-variable time series prediction task in stock movement prediction~\cite{gruver2023large}.




==> kdd_sections/title.tex <==
% \title{PloutosGPT: An Interpretable Quantitative Investment Finance Assistant Evolving With Multi-Strategy Expert System}

\title{PloutosGPT: Towards an Financial Large Language Model for Interpretable Stock Movement Prediction}

==> sections/acknowledgements.tex <==

\section*{Acknowledgments}

The preparation of these instructions and the \LaTeX{} and Bib\TeX{}
files that implement them was supported by Schlumberger Palo Alto
Research, AT\&T Bell Laboratories, and Morgan Kaufmann Publishers.
Preparation of the Microsoft Word file was supported by IJCAI.  An
early version of this document was created by Shirley Jowell and Peter
F. Patel-Schneider.  It was subsequently modified by Jennifer
Ballentine, Thomas Dean, Bernhard Nebel, Daniel Pagenstecher,
Kurt Steinkraus, Toby Walsh, Carles Sierra, Marc Pujol-Gonzalez,
Francisco Cruz-Mencia and Edith Elkind.


==> sections/ethical.tex <==
\section*{Ethical Statement}

There are no ethical issues.
